Towards Bridging the Gap between High-Level Reasoning and Execution on Robots

When reasoning about actions, e.g., by means of task planning or agent programming with Golog, the robot's actions are typically modeled on an abstract level, where complex actions such as picking up an object are treated as atomic primitives with deterministic effects and preconditions that only depend on the current state. However, when executing such an action on a robot it can no longer be seen as a primitive. Instead, action execution is a complex task involving multiple steps with additional temporal preconditions and timing constraints. Furthermore, the action may be noisy, e.g., producing erroneous sensing results and not always having the desired effects. While these aspects are typically ignored in reasoning tasks, they need to be dealt with during execution. In this thesis, we propose several approaches towards closing this gap.

==> diagnosis.tex <==
\chapter{Diagnosis}
\begin{copied}{\cite{haberingUsingPlatformModels2021}}
\section{Approach}\label{sec:approach}

\begin{figure*}[thb]
%\includegraphics[width=\textwidth]{images/pipeline.png}
  \includestandalone[width=\textwidth]{figures/diagnosis-pipeline}
\caption{The diagnosis pipeline, starting with a detected fault and ending with a repair attempt.}
\label{fig:pipeline}
\end{figure*}

%The method we want to propose for a guided explanatory diagnosis generation introduces several requirements to the overall design of the agent. First of all, since diagnosis candidates are generated using existing planning algorithms, we have to fulfil the requirements for these planning algorithms. Specifically, the agent needs to maintain a set of facts about the world, which we call the \textit{world model}. Additionally, the agent requires information about the conditions and effects of each action that it can perform. These action descriptions, together with a list of all available object types and predicates, are collected in the \textit{domain model} and are typically provided using the \textit{PDDL} \todo{Cite PDDL Paper} language. In \autoref{lst:example}, the \emph{PDDL} model of a \emph{move} action is shown, that changes the \emph{(at ?robot ?location)} predicate in the world state for a given current location \emph{?from} to a target location \emph{?to}.

\begin{lstlisting}[float,caption={PDDL definition of a move action},label=lst:example]
(:action move
 :parameters (?r - robot
              ?from - location ?to - location)
 :precondition (at ?r ?from)
 :effect (and (not (at ?r ?from)) (at ?r ?to))))
\end{lstlisting}

The goal is to find a unique explanation for observed faults for two reasons:
\begin{enumerate*}[label=(\alph*)]
\item to regain a consistent belief state, and
\item to recover from any faults
that may have occurred.
\end{enumerate*}
An overview of the approach is shown in
\autoref{fig:pipeline}.

After executing an action sequence and making any observation that contradicts the expected world state, we use the history of executed actions and a model of the underlying hardware platform to generate alternated
histories that explain the observations and thus result in a consistent belief.
In order to do so, we first model the robot platform using finite state
machines, which we then use to model action variants that depend on an
unexpected state of a platform component. We assume that faults are independent
and at least some of them are recoverable. Next, we generate a PDDL domain from
a previously prepared template (containing all actions, possible variants, and the platform model) that
enforces the executed action history (or a variant thereof), which can then
be used with a planner to generate explanation candidates for the observation.
Note that any intermediate observations can be incorporated into the executed
action history as exogenous actions which only assert the observed fact as
effect. This includes any self-diagnostic information gathered by the platform
components, which are modeled as exogenous component state transitions. Once we have
obtained a set of explanation candidates, we use active diagnosis to determine
the most informative sensing action. That sensing action is executed and any
explanation candidates that contradict its sensing result are removed. This is a useful approach in scenarios where we can assume that the execution of sensing actions does not lead to more serious failures. We
continue with the next sensing action until we have a unique explanation
candidate or no other sensing action is possible. In this work, we assume perfect sensing in the context of active diagnosis, however in general active diagnosis is able to cope with sensing noise as well. Finally, based on that
explanation, we update the agent's world model and try to recover from the
fault. If this is not possible, the robot disables itself and asks a human for
help.



%We do this by encoding the constraints given by the platform
%models and the sequence of executed actions into the PDDL domain, formulating
%the problem of finding possible diagnosis candidates as planning problem and
%solving it using existing planning algorithms. If we end up with multiple
%diagnosis candidates, we want to perform active diagnosis to sense for
%literals, that will rule out diagnosis candidates. We integrate knowledge about
%the probabilities of different hardware failures into the active diagnosis
%process in order to evaluate the likelihood of different diagnosis candidates.
%Finally, the active diagnosis should result in a single, valid explanation,
%which allows the agent to deduct a world state that is consistent with the
%observed failure. Due to the integration of hardware models into the diagnosis
%process, possible underlying hardware component failures are part of the
%diagnosis candidates. Therefore, after determining the single valid diagnosis,
%the agent gains additional knowledge about the state of the hardware platform
%it is running on. If possible, the agent can then try to repair the hardware
%failure or decide that it is not operational any more, which is especially
%useful in teams of robots, where the non-operational agent otherwise might
%block resources.

\subsection{Hardware Platform Model}\label{sec:platform}

\begin{figure}
  \centering
  \begin{subfigure}[t]{0.58\linewidth}
    \centering
    \begin{tikzpicture}[
      every node/.append style={font=\tiny},
      state/.append style={rectangle,draw=black,thick,rounded corners},
      edgelabel/.append style={font=\scriptsize\ttfamily},
      exog/.style={dashed},
      ->
      ]
      \node[state] (init) {INIT};
      \node[state,above right=5ex and 4.8em of init] (stuck) {STUCK};
      \node[state,below=5ex of stuck] (broken) {BROKEN};
      %\node[state,below=5ex of init] (locked) {LOCKED};
      \path[exog] (init) edge[bend left] node[edgelabel,midway,above left,align=center] {get-stuck()\\$p=0.25$} (stuck);
      \path (stuck) edge node[edgelabel,pos=0.4,below,sloped] {back-up()} (init);
      \path[exog] (stuck) edge node[edgelabel,midway,right,align=center] {break()\\$p=0.1$} (broken);
      \path[exog] (init) edge node[edgelabel,midway,below,align=center] {break()\\$p=0.1$} (broken);
      %\path[exog] (init) edge[bend right] node[edgelabel,midway,left,align=center] {lock()\\$p=0.12$} (locked);
      %\path[exog] (locked) edge[bend right] node[edgelabel,near start,right] {unlock()} (init);
      %\path[exog] (locked) edge[bend right] node[edgelabel,midway,below right,align=center] {break()\\$p=0.1$} (broken);
    \end{tikzpicture}
    \caption{Navigation}
    \label{fig:navigation}
  \end{subfigure}
  %\hfill
  \begin{subfigure}[t]{0.41\linewidth}
    \centering
    \begin{tikzpicture}[
      every node/.append style={font=\tiny},
      state/.append style={rectangle,draw=black,thick,rounded corners},
      edgelabel/.append style={font=\scriptsize\ttfamily},
      exog/.style={dashed},
      ->
      ]
      \node[state] (init) {INIT};
      \node[state,below=5ex of init] (localized) {LOCALIZED};
      \node[state,below=5ex of localized] (lost) {LOST};
      \path (init) edge node[edgelabel,midway,right] {localize()} (localized);
      \path[exog] (localized) edge[bend right] node[edgelabel,midway,left,align=center] {lost()\\$p=0.05$} (lost);
      \path (lost) edge[bend right] node[edgelabel,midway,right] {localize()} (localized);
    \end{tikzpicture}
    \caption{Localization}
    \label{fig:localization}
  \end{subfigure}
  \caption{Models of the robot hardware components}
  \label{fig:component-models}
\end{figure}

We model the components of the robot platform, e.g., its navigation unit, based
on finite state machines, similar to
\cite{hofmannConstraintbasedOnlineTransformation2018}.  We use two types of
edges:
\begin{enumerate*}[label=(\alph*)]
  \item action edges that the agent can decide to execute, e.g.,
    |localize()| to trigger the localization unit to re-initialize, and
  \item exogenous event edges that are triggered by the environment,
    e.g., |lost()|, which causes the localization unit to lose its known
    pose.
\end{enumerate*}
%
We also attach a probability to each exogenous edge which will be used during active diagnosis to
assign probabilities to the explanation candidates and to determine the most
promising sensing action.

Two example components that are used by the |move| action are shown in
\autoref{fig:component-models}.  \autoref{fig:navigation} shows the navigation
unit of the robot. By default, it is in the state |INIT| (we simplify
the navigation and do not distinguish whether it is currently idle or moving).
However, it may get stuck, e.g., because it hits an obstacle. If that is the
case, the agent can abort the current navigation goal and decide to back up,
which sets the navigation back to the |INIT| state. Similarly, the
navigation may suffer from a hardware failure, which completely blocks the
movement and from which the agent cannot recover.
The localization unit in \autoref{fig:localization} first needs to be
initialized with the |localize()| action. While it is in use, it
sporadically gets |lost()|, in which case it needs to be re-initialized
with another |localize()| action.

\begin{lstlisting}[float,caption={An exogenous state transition action in PDDL},label=lst:get-stuck]
(:action get-stuck
 :parameters ()
 :precondition (state NAVIGATION INIT)
 :effect (and (not (state NAVIGATION INIT))
              (state NAVIGATION STUCK))
              (increase (total-cost) 1)))
\end{lstlisting}

\begin{lstlisting}[float,caption=An action with hardware component constraints,label=lst:complete_move]
(:action move
 :parameters (?r - robot
              ?from - location ?to - location)
 :precondition (and (at ?r ?from)
                    (state NAVIGATION INIT)
                    (state LOCALIZATION LOCALIZED))
 :effect (and (not (at ?r ?from)) (at ?r ?to)))
\end{lstlisting}

\subsection{Creating a PDDL Diagnosis Domain}\label{sec:domain}
With the goal to take a \emph{diagnosis as planning} approach, we generate a
PDDL domain that completely describes the diagnosis problem. We do this by
\begin{enumerate*}
  \item adding the nominal platform state to the precondition of actions,
  \item adding actions for the exogenous events, following the platform model,
  \item providing action variants of the original actions, depending on faulty
    states of the platform, and
  \item enforcing the history, i.e., any solution of the problem must include
    each action (or one of its variants) of the originally executed plan.
\end{enumerate*}

In order to incorporate the platform model into the PDDL domain, we model the
component states as PDDL domain objects and the current states as PDDL predicates
|(state ?c - component ?s - state)|.
Furthermore, we add exogenous events as PDDL actions, as
shown in \autoref{lst:get-stuck} for the |get-stuck| transition of the
navigation component. Using these PDDL platforms models, we can model the
dependencies of the available actions on the hardware components. For example,
the move action as defined in \autoref{lst:example} depends on the navigation
component as well as the localization component, as defined in
\autoref{fig:component-models}. Therefore, we add preconditions for the required
states of the component models to the PDDL model of the move action, as shown in
\autoref{lst:complete_move}.

\subsubsection{Creating Action Variants}

In general, an action variant models a fault mode of an action in the
original domain.  While these are typically written ad-hoc based on the
experience with failed execution runs, our platform models allow a more
principled approach: As we have already added the expected state of a platform
component to the original action, we can now also define an action variant
for each state that the platform component may have reached by exogenous
events.  For example, the navigation component in
\autoref{fig:navigation} contains an exogenous transition from the
|INIT| state to the |STUCK| state, which represents the situation
that the robot is not able to move. Therefore, as shown in
\autoref{lst:move-stuck}, we add an action variant |move-stuck| of the
action |move| that models the behavior of the action if the navigation
is stuck. In |move-stuck|, the precondition is adapted to require the
navigation to be stuck. The effect models what happens if the robot executes a
|move| action while it is stuck, which is nothing in this case.
In order to ensure that the diagnosis process is able to determine the effects
of all hardware faults that might have happened, it is beneficial to use the
hardware models as a guide. Although different hardware faults may result in the
same action variant, using the possible platform states as a guideline to create
all variants will result in a complete description of the faulty behaviour.

%It might happen that the agent executes an action, because it assumes the
%dependent hardware components to be in the required states, while in reality
%one of the components has transitioned to another, faulty state, without being
%recognized by the agent. In order to enable the diagnosis generation process
%reason about the different possible outcomes of an action that was executed
%without all component dependencies being fulfilled, we have to model the
%possible faulty action variants. As a guideline, we can use the existing
%hardware component dependencies. For example, the \emph{move base} component
%model contains an exogenous transition from the \emph{INIT} state to the
%\emph{STUCK} state, which represents the situation that the robot is not able
%to move. Therefore, the diagnostic generation process requires an action
%variant of the \emph{move} action for the states that are reachable via
%exogenous transitions.

\begin{lstlisting}[float,caption=A faulty variant of the move action,label=lst:move-stuck]
(:action move-stuck
 :parameters (?r - robot ?from - location)
 :precondition (and (at ?r ?from)
                    (state NAVIGATION STUCK)
                    (state LOCALIZATION LOCALIZED))
 :effect ())
\end{lstlisting}

\begin{lstlisting}[float,caption=Order action template,label=lst:order_action_template]
(:action order-i
 :parameters ()
 :precondition (last-ACT_i PARAM_i)
 :effect (and (not (last-ACT_i PARAM_i))
                (next-ACT_i+1 PARAM_i+1)))
\end{lstlisting}

\subsubsection{Enforcing the History}

We are not merely interested in any sequence of
actions that is an explanation for the observation but rather only in action
sequences that represent an adapted version of the original action sequence.
For example, suppose an agent that executed the actions \textsc{A} and \textsc{B}, starting
from a world state \textsc{s}, and observes the contradicting fact \textsc{f}. A
planner might determine a plan consisting of the single action \textsc{C} as
possible diagnosis. However, this does not take into account
that the agent executed \textsc{A} and \textsc{B}. The only valid
explanations are therefore sequences of actions that consist of variants of
\textsc{A} and \textsc{B} and insertions of exogenous actions.  Thus, we need
to forbid solutions that do not result from possible variants of the original
action sequence. We do this with \emph{order actions}, which force the planner
to insert variants of the executed actions in the right order.

\begin{lstlisting}[float,caption=Grounded order action to enforce \texttt{grab} after
\texttt{move},label=lst:order_action]
(:action order-1
 :parameters ()
 :precondition (last-move R1 C-BS C-CS1)
 :effect (and (not (last-move R1 C-BS C-CS1))
                (next-grab R1 WP1 C-CS1))
\end{lstlisting}

\begin{lstlisting}[float,caption=A non-faulty action with order predicates.,label=lst:standard_action]
(:action move
 :parameters (?r - robot
              ?from - location ?to - location)
 :precondition (and (next-move ?r ?from)
                    (at ?r ?from))
 :effect (and (not (at ?r ?from)) (at ?r ?to)
              (not (next-move ?r ?from))
                   (last-move ?r ?from))))
\end{lstlisting}

For a given action sequence $h = \lbrace a_1, \ldots , a_n \rbrace $, we add an
action |order-i| for each $a_i$, as shown in
\autoref{lst:order_action_template}, where
|ACT_i| is replaced with the action type of $a_{i}$ and
  %and |ACT_i+1| with the action type of $a_{i+1}$.
|PARAM_i| is replaced with parameters of $a_{i}$.
  %The same applies to |PARAM_i+1|.
We replace |ACT_0| by |BEGIN| and |ACT_n+1| by |FINISHED|, where |(last-BEGIN)| is
true initially and |(next-FINISHED)| is part of the goal. An example for such an order
action
%that follows a move of robot R1 from C-BS to C-CS1 and precedes a grab
%of WP1 from C-CS1,
is shown in \autoref{lst:order_action}. We also add a new
precondition and a new effect to each action and its variants to enforce the
order actions, as shown exemplarily for the |move| action in
\autoref{lst:standard_action}.

To reach a goal state, in which |(last-FINISH)| holds, the planner has
to generate a sequence of the form $h' = \{o_0,a'_1,o_1, \ldots , a'_n, o_n
\}$, where $o_i$ is an order action and $a'_j$ is either $a_j \in h$ or one of
its faulty variants. Additional exogenous actions may be inserted anywhere in the sequence.

\subsubsection{Action Variants Based on Changing Parameters}
With the construction above, we can force any diagnosis produced by a planner to
form a variant of the original action sequence, including the actions'
parameters. However, when executing an action, the action's parameters may
change without being noticed by the executive, thereby producing
another variant of the action. Instead of specifying those variants
explicitly, we obtain them by only fixing some of the parameters in the
|(last-...)| and |(next-...)| predicates.
In order to do so, we have to differentiate between parameters that
would have caused the execution to fail in the first place if changed, and
parameters that may change unknowingly.

Consider a |move| action that takes as argument the current position |?from| of
the robot and the target machine |?to|.  Assuming that the execution will fail
if the robot is not actually starting from where it expects to be, then the
starting position cannot have changed unnoticed. Therefore, |?from| has to be
enforced by the |order| predicates.  On the other hand, the robot might not end
up where it expected, e.g., if the target machine was moved from its
original location. In order to enable the diagnosis process to consider this
possibility, the |?to| parameter should be replacable and not be part
of the |order| predicates, as shown in \autoref{lst:standard_action}. The
decision about which parameters have to be enforced in the history depends on
the specific implementation and execution of the actions and can differ from
platform to platform.

\begin{lstlisting}[float,caption=A put action with conditional effect. Hardware dependencies and order predicates are removed for visibility purposes., label=lst:cond_action]
(:action put
 :parameters (?r - robot
              ?mps - location ?wp - workpiece)
 :precondition (at ?r ?mps)
 :effect (and (when (holds ?r ?wp)
                    (and (not (holds ?r ?wp))
                         (at ?wp ?mps)))))
\end{lstlisting}

\subsubsection{Action Variants Based on Conditional Effects}
When designing the PDDL definition of an action with the intention to use
it for planning, it is sufficient to model the effects and preconditions of an
action without any faults in mind. However, when executed on a real robot, an
action's precondition may not be satisfied and still execute
successfully, but only achieving its effects partially. As an example, if the
robot executes |put| while not actually holding a workpiece, the execution may
succeed (assuming it is not equipped with an appropriate sensor), but without
the expected effects, as the workpiece will not be on the machine. Therefore,
for diagnosis purposes, the
effect needs to be modelled as conditional effect, depending on whether the
robot is holding the workpiece. The corresponding PDDL action with this
conditional effect is shown in \autoref{lst:cond_action}.
%
Additionally, an action may also have undesired side effects, e.g., if
there was already a workpiece on the machine before the robot executed |put|, it
may knock that workpiece from the machine.
%
Modelling those conditional and side effects is crucial for
diagnosis, as only then the diagnosis process will be able to determine all
possible outcomes of an action. Based on our experiences, we have identified some principles for modelling
actions for diagnosis purposes:
\begin{enumerate*}
\item The precondition must express the necessary condition
  for the action not to fail completely during execution.
\item Any other condition, which changes the effect of the action but does not
  affect its executability, must be used as a condition of a conditional
  effect.
\item An action may have additional side effects on other
  objects. Such effects need to be added as conditional effect and possibly
  require the other objects as additional parameters of the action.
\end{enumerate*}

\subsubsection{Generating the PDDL Domain and Problem Description}
We conclude this section by summarizing the process of generating the PDDL
domain and problem description for a particular diagnosis problem.
We start with a PDDL domain augmented by exogenous actions, action variants,
and modified action preconditions that require the respective platform states,
as described above.  For a given initial state, an action history $h = \{a_1 ,
\ldots , a_n\}$, and a set of
observations, we generate the PDDL description as follows:
\begin{enumerate}
\itemsep-0.1em
\item For each $a_i$, insert an order action $o_i$ into the domain.
  %for each $i \in \{0, \ldots, n\}$;
\item As initial state of the problem, use the state in which $h$ started (i.e.,
  the initial state of the original plan).
\item Add |(next-BEGIN)| to the initial state to fulfill the precondition
  of the first order action $o_0$.
\item Create the goal formula as a conjunction of the observed fault
  and |(last-FINISH)| to enforce the complete history $h$.
\end{enumerate}

The resulting PDDL domain and problem description can then be used to determine
possible diagnoses.

\subsection{Top-$k$ Planning for Diagnosis Generation}\label{sec:top-k}
With the generated PDDL domain and problem description, we
can use a PDDL planner to determine a possible history alternative that
explains the observations. As we are interested in
multiple explanation candidates, we will use a top-$k$ planner
\cite{katzNovelIterativeApproach2018} that generates $k$ cost-optimal solutions.
As metric, we apply Ockham's razor and assume that diagnoses with fewer exogenous
actions are more likely. We achieve this by applying a cost of $1$ to each
exogenous action, while each plan action (and its variant) have a cost of $0$.
By doing so, we will obtain explanations with the least possible amount of
faults. It is possible that the real explanation contains more faults
than other possible explanations and might not be included in the first $k$
plans. However, since there might be an infinite number of possible explanations,
we fix $k$ such that the risk of missing the real explanation is negligible.

%Equipped with models of all required action failures, as indicated by the
%hardware platform model, we can try to generate possible explanations for any
%sensed failure. As mentioned before, in history-based diagnosis a diagnosis
%candidate is a modification of the sequence of executed actions by inserting
%exogenous actions or replacing executed actions with faulty variants. We want
%to use existing planning algorithms in order to efficiently generate all needed
%possible explanations.
%
%The K* planner\todo{Do we really use K*? Katz et al.\ is not K*}
%is a top-\textit{k} planner, which generates \textit{k} plans
%for a given initial world state, a domain description, a goal and a metric. A
%plan consist of a sequence of grounded actions, that lead from the initial
%world state to a world state in which the goal condition is fulfilled. It is
%guaranteed, that there is exist no solution with a better metric than any of
%the \textit{k} plans, which is not already part of the \textit{k}-set. We want
%to encode the problem of finding the most likely suitable action sequence
%variants for a given contradicting observation as a PDDL planning problem in
%order to utilize the K* planner. As a metric we want to incorporate Ockham's
%razor by introducing a cost of 1 to each exogenous action representing a fault.
%By minimizing the sum of all exogenous actions, the K* planner primarily
%generates explanations with the least amount of assumed faults.

\subsection{Active Diagnosis}\label{sec:active-diagnosis}
Starting with a set of possible explanations generated by the top-$k$ planner,
we now determine which of those is the correct one.
However, before we continue with excluding possible diagnosis candidates with
active diagnosis, we filter this set of $k$ possible solutions by
excluding one of any two diagnosis candidates that would result in the same
world state. To result in the same world state,
two diagnosis candidates have to contain the same component faults.
For example, if a possible solution for the given problem would be
the insertion of an exogenous action $e$ into the sequence, then the planner
would treat all solutions that has $e$ inserted at any place in the sequence as
distinct solutions, even though some of them might result in exactly the same state.
As we cannot distinguish those explanations, we only keep one of them.

Next, we apply \emph{active diagnosis} to filter the explanation
candidates.  For a given set of candidates, we determine the common set of
facts, the so-called \emph{shared
knowledge}.  For every candidate that can be excluded by a sensing action, the
shared knowledge will increase, as at least one disagreement on a fact will be
resolved.  Following %the active diagnosis approach by
\cite{muhlbacherActiveDiagnosisAgents2014}, we select the sensing
action with the highest impact on the set of diagnosis candidates.

For a set of diagnosis candidates $D$ and a grounded sensing action $a$ that senses
whether a predicate $f$ is true, the action $a$ splits $D$ into $D_+$ and $D_-$.
The subset $D_+$ contains all diagnosis candidates that are consistent with a positive
outcome of $a(\vec{x})$ and $D_-$ all candidates that are consistent with a
negative outcome.
%
Using the combined probabilities $p_{D_+} = \sum_{d \in D_+} p_d$
(similarly for $p_{D_-}$), we can calculate the entropy of
$a$, which is a metric for the impact of $a$ onto $D$:
\begin{equation*}
  E(D,a) = -\left( p_{D_p} \log_2 p_{D_p} + p_{D_n} \log_2 p_{D_n} \right)
\end{equation*}
To determine the probability $p_d$ of a single diagnosis candidate $d$, we
combine the probability of all exogenous actions $F_d$ that are part of the
diagnosis candidate $d$: $p_d = \prod_{f \in F_d} p_f$.  Since exogenous actions
represent exogenous event edges of a hardware component model, we can directly
use the probabilities assigned to these exogenous edges.  Therefore, the
engineering knowledge encoded in the platform model directly affects the
selection of the sensing action.

After repeatedly using active diagnosis to determine the sensing action with the highest impact, executing
the action, and excluding mismatching diagnosis candidates, the agent
ends up with one or more remaining diagnosis candidates. Finally, the agent can integrate all facts that are true
in all remaining diagnosis candidates into its world model. %, since these facts hold true for each possible explanation.
Similarly, it can remove all facts that are inconsistent with all remaining diagnosis candidates.
Next, it can try to repair any hardware component that was determined to be
faulty.
%Any hardware component whose state was updated due to the diagnosis can then be tried to repair.
If this is not possible, it may decide to call for human intervention
or disable itself, since the robot is not operable any more.

\section{Evaluation}\label{sec:diagnosis-evaluation}

\begin{table}
  \centering
  \fontsize{9}{10}\selectfont
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{l r r r  r r r  r r r}
    \toprule
    $p_\text{failure}$ & \multicolumn{3}{c}{\SI{0.12}{\percent}} &
    \multicolumn{3}{c}{\SI{0.19}{\percent}} & \multicolumn{3}{c}{\SI{0.27}{\percent}}
    \\
    \cmidrule(r){1-1}\cmidrule(rl){2-4} \cmidrule(rl){5-7} \cmidrule(l){8-10}
    & $\emptyset$ & D & DP
    & $\emptyset$ & D & DP
    & $\emptyset$ & D & DP
    \\
    \midrule
    \# Plans & 1874 & 1136 & 2102 & 1527 & 683 & 3312 & 2019 & 542 & 3766
    \\
    ~~\# Failed & 527 & 288 &  115 & 621 & 165 & 121 & 757 & 219 & 379
    \\
    ~~\% Failed  & 28.1 & 25.3 & 5.5 & 40.6 & 24.1 & 3.6 & 37.5 & 40.4 & 10.1
    \\
    \# Diagnoses & 0 & 56 & 49 & 0 & 20 & 66 & 0 & 22 & 111
    \\
    \# Repairs & 0 & 0 & 31 & 0 & 0 & 38 & 0 & 0 & 69
    \\
    \# Disabled & 0 & 0 & 26 & 0 & 0 & 32 & 0 & 0 & 50
%    \\
%    Diagnosis time
%    \\
%    \: mean (\si{\second}) & & 3.54 & 3.97 & & 5.45 & 4.52 & & 3.91 & 4.05
%    \\
%    \: stddev (\si{\second}) & & 1.38 & 1.72 & & 2.19 & 1.59 & & 1.80 & 1.87
    \\
    \bottomrule
  \end{tabular}
  \caption{The number of plans, diagnoses, repairs, and robot disengagements in
  the simulated RCLL games, where $\emptyset$ stands for \emph{no diagnosis}, D
for \emph{diagnosis without platform models}, and DP for \emph{diagnosis with
platform models}.}
  \label{tbl:eval-overview}
\end{table}

\begin{table}
%\ra{2}
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{r rrr rrr rrr}
\toprule
 & \multicolumn{3}{c}{Game Score} & \multicolumn{6}{c}{Game Score w/ Diagnosis} \\
 %\cmidrule{6-12}
 & \multicolumn{3}{c}{w/o Diagnosis} & \multicolumn{3}{c}{w/o platform} & \multicolumn{3}{c}{w/ platform}\\
 \cmidrule(rl){2-4} \cmidrule(rl){5-7}  \cmidrule(l){8-10}
 $p_{\text{failure}}$
& Mean & Min & Max & Mean & Min & Max & Mean & Min & Max \\
\midrule
    $0.12\%$ & 71.31 & 6 & 260 & 76.66 & 12 & 217 & 160.94 & 93 & 229 \\
%\midrule
    $0.19\%$ & 58 & 4 & 142 & 68.44 & 12 & 151 & 156.6 & 91 & 295\\
%\midrule
    $0.27\%$ & 32.75 & 0 & 98 & 37.88 & 0 & 144 & 109.5 & 10 & 174 \\
\bottomrule
  \end{tabular}
\caption{Game scores in simulated RCLL games of a team of robots without
diagnosis, with diagnosis but without platform models, and with diagnosis
including platform models. Failure was simulated, $p_\text{failure}$ is the
probability of a failure in an interval of \SI{1}{\second}.}
\label{points_table}
\end{table}


We implemented the proposed diagnosis approach\footnote{The code is open
  source and available at
\mbox{\url{https://github.com/Sagre/GuidedExplanatoryDiagnosis}}.}
and integrated it into the goal reasoning system CLIPS
Executive~\cite{niemuellerGoalReasoningCLIPS2019}.
% TODO add ref to rulebook
We evaluated our approach in a scenario from the RoboCup Logistics League (RCLL)
\cite{niemuellerRoboCupLogisticsLeague2016,hofmannMultiagentGoalReasoning2021}.
In the RCLL, a team of three robots needs to operate machines to manufacture
products. In order to do so, a robot needs to
put workpieces on and grab workpieces from machines, and instruct the machines
to process the workpiece. A team scores points upon successful delivery of a
product.

We modeled the gripper, RGB/D camera, and RGB camera
as hardware components. The gripper may become
decalibrated or break completely. Also, the gripper's fingers may get
stuck. Each camera might crash, which sometimes can be repaired by performing a reset.
We extended an implemenation of the RCLL in the Gazebo simulator
\cite{zwillingSimulationRoboCupLogistics2014} with simulated
failures of each of those components.

We simulated full RCLL games with simulated failures with diagnosis including
platform models and compared it to diagnosis without platform models and no
diagnosis at all. Both approaches try to recover a valid world model after observing an action failure. In cases where this is successful, the agents will try to continue the operation. \autoref{tbl:eval-overview} shows a summary of the results. We
can see that with diagnosis, the percentage of successful plans increases. We
can also see that diagnosis with platform models considerably outperforms
diagnosis without platform models, for several reasons:
%First, diagnosis is successful more often because the diagnosis process has more information.
First, even with a successful diagnosis, the system without platform models
cannot find a repair action, because there is no known underlying cause; the
action variant seems to have occurred randomly. In contrast, with platform
models, the underlying reason (a failed platform component) can be diagnosed and
repaired. Second, with platform models, the robot is able to detect
when it is no longer operational, e.g., because its gripper is broken. In this
case, it can disengage and stop interfering with the other robots.
\autoref{points_table} shows the game scores in each configuration. As we can
see, diagnosis with platform models increases the team's score significantly,
especially in configurations where faults occur more often.
Considering the running time $t$, both approaches perform similarly,
with $t = \SI{4.00 \pm 1.80}{\second}$ for diagnosis without platform models
and $t = \SI{4.17 \pm 1.76}{\second}$ for diagnosis with platform models.

\end{copied}


